Searching for Extragalactic Exoplanetary Systems: the Curious Case of BD+20 2457

Planets and their host stars carry a long-term memory of their origin in their chemical compositions. Thus, identifying planets formed in different environments improves our understating of planetary formation. Although restricted to detecting exoplanets within the solar vicinity, we might be able to detect planetary systems that formed in small external galaxies and later merged with the Milky Way. In fact, Gaia data have unequivocally shown that the Galaxy underwent several significant minor mergers during its first billion years of formation. The stellar debris of one of these mergers, Gaia-Enceladus (GE), is thought to have built up most of the stellar halo in the solar neighborhood. In this Letter, we investigate the origin of known planet-host stars combining data from the NASA Exoplanet Archive with Gaia EDR3 and large-scale spectroscopic surveys. We adopt a kinematic criterion and identify 42 stars associated with the Milky Way's thick disk and one halo star. The only halo star identified, BD+20 2457, known to harbor two exoplanets, moves on a retrograde and highly eccentric orbit. Its chemical abundance pattern situates the star at the border between the thick disk, the old halo, and accreted populations. Given its orbital parameters and chemical properties, we suggest that BD+20 2457 is likely formed in the protodisk of the Galaxy, but we do not exclude the possibility of the star belonging to the debris of GE. Finally, we estimate a minimum age and mass limit for the star, which has implications for its planetary system and will be tested with future Transiting Exoplanet Survey Satellite observations.

==> table.tex <==


\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{0.30em}

%\newpage 


%\begin{landscape}
\begin{longrotatetable}
\begin{ThreePartTable}
\begin{TableNotes}
\scriptsize
\item[] Notes: 
\item[]The symbols $\dagger$ ({\it Gaia}), $\ddagger$ (APOGEE), $\star$ (GALAH), $\S$ (LAMOST) indicates the catalog from where the RV, [Fe/H], $T_{\rm eff}$, log $g$ were obtained. 
\item[] (a) Classified as thick disk star according to our kinematical criterion.
\item[] (b) Classified as thick disk star according to both kimematical criteria: our and \cite{bensby2003} adapted formalism (Appendix \ref{app:formalism}). Stars with $TD/D > 10$ are classified as thick disk.
\end{TableNotes}


\footnotesize

\begin{longtable}{>{\scriptsize}l >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c
>{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c >{\scriptsize}c}

\caption{Table of planet--host stars classified as halo or thick disk stars} \label{tab:long} \\

\hline \multicolumn{1}{>{\scriptsize}l}{Star Name} & \multicolumn{1}{>{\scriptsize}c}{{\it Gaia} EDR3 ID} & \multicolumn{1}{>{\scriptsize}c}{R.A.} & \multicolumn{1}{>{\scriptsize}c}{Decl.} & \multicolumn{1}{>{\scriptsize}c}{Distance} & \multicolumn{1}{>{\scriptsize}c}{RV} & \multicolumn{1}{>{\scriptsize}c}{[Fe/H]} & \multicolumn{1}{>{\scriptsize}c}{$T_{\rm eff}$} & \multicolumn{1}{>{\scriptsize}c}{$\log g$} & \multicolumn{1}{>{\scriptsize}c}{Class.} & 
\multicolumn{1}{>{\scriptsize}c}{$E$} & \multicolumn{1}{>{\scriptsize}c}{$L_z$}& \multicolumn{1}{>{\scriptsize}c}{Ecc} & \multicolumn{1}{>{\scriptsize}c}{($v_R$, $v_{\phi}$, $v_z$)}& 
\multicolumn{1}{>{\scriptsize}c}{$Z_{\max}$} & \multicolumn{1}{>{\scriptsize}c}{$R_{apo}$} & \multicolumn{1}{>{\scriptsize}c}{$R_{peri}$} \\

%
& & & & & & & & & & \multicolumn{1}{>{\scriptsize}c}{$\times 10^5$} &  \multicolumn{1}{>{\scriptsize}c}{$\times 10^3$} & & & & & \\ 
%

 &  & \multicolumn{1}{>{\scriptsize}c}{deg} & \multicolumn{1}{>{\scriptsize}c}{deg} & \multicolumn{1}{>{\scriptsize}c}{kpc} & \multicolumn{1}{>{\scriptsize}c}{km\,s$^{-1}$} & \multicolumn{1}{>{\scriptsize}c}{dex} & \multicolumn{1}{>{\scriptsize}c}{K} & \multicolumn{1}{>{\scriptsize}c}{cgs} &  
 &
 \multicolumn{1}{>{\scriptsize}c}{km$^2$ s$^{-2}$}  & \multicolumn{1}{>{\scriptsize}c}{kpc\,km\,s$^{-1}$} &
                     & 
\multicolumn{1}{>{\scriptsize}c}{km\,s$^{-1}$} &
\multicolumn{1}{>{\scriptsize}c}{kpc}              & 
\multicolumn{1}{>{\scriptsize}c}{kpc} & 
\multicolumn{1}{>{\scriptsize}c}{kpc}  \\ 

\hline \hline 
\endfirsthead

\multicolumn{17}{c}%
{{\tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{>{\scriptsize}l}{Star Name} & \multicolumn{1}{>{\scriptsize}c}{{\it Gaia} EDR3 ID} & \multicolumn{1}{>{\scriptsize}c}{RA} & \multicolumn{1}{>{\scriptsize}c}{DEC} & \multicolumn{1}{>{\scriptsize}c}{Distance} & \multicolumn{1}{>{\scriptsize}c}{RV} & \multicolumn{1}{>{\scriptsize}c}{[Fe/H]} & \multicolumn{1}{>{\scriptsize}c}{$T_{\rm eff}$} & \multicolumn{1}{>{\scriptsize}c}{log $g$} & \multicolumn{1}{>{\scriptsize}c}{Class.} & 
\multicolumn{1}{>{\scriptsize}c}{$E$} & \multicolumn{1}{>{\scriptsize}c}{$L_z$}& \multicolumn{1}{>{\scriptsize}c}{Ecc} & \multicolumn{1}{>{\scriptsize}c}{($v_R$, $v_{\phi}$, $v_z$)}& 
\multicolumn{1}{>{\scriptsize}c}{$Z_{\max}$} & \multicolumn{1}{>{\scriptsize}c}{$R_{apo}$} & \multicolumn{1}{>{\scriptsize}c}{$R_{peri}$} \\

%
& & & & & & & & & & \multicolumn{1}{>{\scriptsize}c}{$\times 10^5$} &  \multicolumn{1}{>{\scriptsize}c}{$\times 10^3$} & & & & & \\ 
%

 &  & \multicolumn{1}{>{\scriptsize}c}{deg} & \multicolumn{1}{>{\scriptsize}c}{deg} & \multicolumn{1}{>{\scriptsize}c}{kpc} & \multicolumn{1}{>{\scriptsize}c}{km\,s$^{-1}$} & \multicolumn{1}{>{\scriptsize}c}{dex} & \multicolumn{1}{>{\scriptsize}c}{K} & \multicolumn{1}{>{\scriptsize}c}{cgs} &  
 &
 \multicolumn{1}{>{\scriptsize}c}{km$^2$ s$^{-2}$}  & \multicolumn{1}{>{\scriptsize}c}{kpc\,km\,s$^{-1}$} &
                     & 
\multicolumn{1}{>{\scriptsize}c}{km\,s$^{-1}$} &
\multicolumn{1}{>{\scriptsize}c}{kpc}              & 
\multicolumn{1}{>{\scriptsize}c}{kpc} & 
\multicolumn{1}{>{\scriptsize}c}{kpc} \\                   
\hline \hline 
\endhead

\hline 
\insertTableNotes  \\
\multicolumn{17}{>{\scriptsize}l}{{Continued on next page}}
\endfoot

% & 1 & 1 & 1 & 1 & 1 & 1 &  1

\hline 
\insertTableNotes \\ 
\endlastfoot
BD+20 2457 & 625137162857354880 & 154.1867 & 19.8912 & 1.44 & 145.7$^{\dagger}$ & & & & Halo & 1.57 & -0.23 & 0.91 & (190.6,-26.4,-53.2) & 6.38 & 0.59 & 12.78
\\
HAT-P-12 & 1499514786891168640 & 209.3886 & 43.4933 & 0.141 & -40.0$^{\dagger}$ & & & & TD (a) & 1.70 & -1.30 & 0.34 & (36.7,158.0,0.5) & 0.15 & 4.16 & 8.41
\\
HAT-P-12 & 1499514786891168640 & 209.3886 & 43.4933 & 0.141 & -46.2$^{\S}$ & -0.26 & 4679 & 4.62 & TD (a) & 1.70 & -1.28 & 0.34 & (36.7,155.7,-5.38) & 0.18 & 4.07 & 8.4 
\\
HAT-P-26 & 3668036348641580288 & 213.1565 & 4.059 & 0.142 & 14.5$^{\dagger}$ & & & & TD (a)
& 1.61 & -1.56 & 0.30 & (-86.7,191.5,-26.3) & 0.50 & 5.10 & 9.65
\\
HAT-P-26 & 3668036348641580288 & 213.1565 & 4.059 & 0.142 & 10.9$^{\S}$ & 0.03 & 5090 & 4.48 & TD (a) & 1.61 & -1.56 & 0.30 & (-85.1,191.9,-29.1) & 0.56 & 5.13 &  9.61
\\
HD 111232 & 5855730584310531200 & 192.2160 & -68.4247 & 0.029 & 104.5$^{\dagger}$ & & & & TD (a) & 1.67 & -1.34 & 0.36 & (-71.6,163.1,-12.6) & 0.19 & 4.19 &  8.94
\\
HD 11755 & 558504529130235136 & 29.7078 & 73.1521 & 0.232 & -87.6$^{\dagger}$ & & & & TD (b) & 1.49 & -1.87 & 0.26 & (-84.9,224.0,-85.6) & 2.72 & 6.71 &  11.49
\\
HD 136418 & 1392396172224832896 & 229.7756 & 41.7323 & 0.104 & -34.2$^{\dagger}$ & & & & TD (a) & 1.65 & -1.45 & 0.32 & (-72.8,177.3,-4.0) & 0.13 & 4.71 &  9.09
\\
HD 233604 & 1023492257121204352 & 137.4535 & 53.5682 & 0.857 & -73.7$^{\dagger}$ & & & & TD (a) & 1.51 & -1.86 & 0.33 & (-107.5,209.9,17.9) & 1.04 & 5.97 & 11.87
\\
HD 233604 & 1023492257121204352 & 137.4535 & 53.5682 & 0.857 & -77.2$^{\S}$ & -0.29 & 4804 & 2.43 & TD (a) & 1.50 & -1.85 & 0.33 & (-110.3,209.1,15.21) & 1.01 & 5.90 &  11.9
\\
HD 47536 & 5583831735369515008 & 99.4489 & 32.3394 & 0.124 & 79.7$^{\dagger}$ & & & & TD (a) & 1.65 & -1.42 & 0.28 & (44.3,171.1,54.9) & 1.24 & 4.87 &  8.64
\\
HD 5583 & 363012289421389056 & 14.4870 & 34.9853 & 0.216 & 11.9$^{\dagger}$ & & &  & TD (a)
  & 1.63 & -1.42 & 0.36 & (89.2,170.1,-36.8) & 0.76 & 4.44 &  9.61
\\
HD 5891 & 2788816827588309120 & 15.1383 & 20.2923 & 0.278 & -96.2$^{\dagger}$ & & & & TD (a)
& 1.66 & -1.34 & 0.35 & (-64.7,161.1,33.2) & 0.67 & 4.26 & 8.98
\\
K2-111 & 53006669599267328 & 59.8903 & 21.2985 & 0.198 & -16.7$^{\dagger}$ & & &  & TD (b)
& 1.69 & -1.24 & 0.34 & (13.9,147.9,67.4) & 1.77 & 4.18 & 8.43
\\
K2-15 & 3896271842760486272 & 178.1106 & 4.2547 & 0.498 & -9.9$^{\S}$ & -0.25 & 5053 & 4.68 & TD (a) & 1.65 & -1.37 & 0.31 & (62.1,167.0,-48.3) & 1.38 & 4.61 &  8.84
\\
K2-166 & 3701015375282968064 & 185.1880 & 2.2823 & 0.479 & -8.7$^{\S}$ & -0.19 & 5915 & 3.93 & TD (a) & 1.64 & -1.44 & 0.29 & (62.6,177.2,-27.9) & 0.82 & 4.85 &  8.85
\\
K2-204 & 2533185974768028032 & 17.3825 & -0.5177 & 0.547 & -50.6$^{\star}$ & -0.10 & 5746 & 4.16 & TD (a) & 1.63 & -1.51 & 0.30 & (-69.2,180.6,16.0) & 0.58 & 5.00 &  9.30
\\
K2-271 & 655863775507590400 & 125.2239 & 16.0908 & 0.538 & -75.9$^{\S}$ & -0.48 & 5496 & 4.17 & TD (a) & 1.54 & -1.68 & 0.36 & (-112.6,194.7,-35.8) & 0.91 & 5.24 &  11.3
\\
K2-86 & 55994798604873216 & 51.5531 & 18.6356 & 0.254 & 122.5$^{\dagger}$ & & & & TD (a)
& 1.51 & -1.78 & 0.39 & (130.9,211.4,-17.4) & 0.37 & 5.38 & 12.40
\\
K2-86 & 55994798604873216 & 51.5531 & 18.6356 & 0.254 & 122.4$^{\star}$ & -0.43 & 5030 & 4.47 & TD (a) & 1.50 & -1.78 & 0.39 & (130.7,211.4,-17.4) & 0.37 & 5.38 &  12.40
\\
K2-86 & 55994798604873216 & 51.5531 & 18.6356 & 0.254 & 115.2$^{\S}$ & -0.30 & 5211 & 4.48 & TD (a) & 1.51 & -1.77 & 0.37 & (123.7,209.8,-13.0) & 0.27 & 5.41 &  11.9
\\
KIC 5437945 & 2102070660978313472 & 288.4750 & 40.6513 & 1.298 & -88.4$^{\S}$ & -0.75 & 7662 & 4.14 & TD (a) & 1.65 & -1.37 & 0.19 & (-10.4,174.0,-89.9) & 2.30 & 5.41 & 8.08
\\
Kepler-10 & 2132155017099178624 & 285.6793 & 50.2415 & 0.186 & -98.1$^{\dagger}$ & & & & TD (a) & 1.71 & -1.26 & 0.36 & (37.2,153.7,1.9) & 0.08 & 3.98 & 8.38
\\
Kepler-10 & 2132155017099178624 & 285.6793 & 50.2415 & 0.186 & -98.6$^{\ddagger}$ & -0.13 & 5685 & 4.50 & TD (a) & 1.71 & -1.26 & 0.36 & (37.3,153.2,1.7) & 0.08 & 3.96 & 8.38
\\
Kepler-10 & 2132155017099178624 & 285.6793 & 50.2415 & 0.186 & -104.1$^{\S}$ & -0.25 & 5623 & 4.18 & TD (a) & 1.71 & -1.21 & 0.37 & (38.0,148.2,0.0) & 0.08 & 3.77 & 8.37
\\
Kepler-112 & 2078722600285671936 & 296.9811 & 43.2097 & 0.511 & -92.3$^{\S}$ & -0.62 & 5484 & 4.11 & TD (b) & 1.66 & -1.38 & 0.23 & (16.7,170.0,-69.2) & 1.68 & 5.01 & 8.17
\\
Kepler-1228 & 2080534148769345408 & 296.5528 & 46.9662 & 0.513 & -89.2$^{\S}$ & -0.39 & 5011 & 4.64 & TD (b) & 1.68 & -1.12 & 0.44 & (-79.7,138.2,66.2) & 1.82 & 3.49 & 8.97
\\
Kepler-1258 & 2132156632006693504 & 285.4049 & 49.9948 & 0.707 & -66.8$^{\S}$ & -0.49 & 5736 & 4.25 & TD (a) & 1.62 & -1.52 & 0.32 & (88.1,186.8,6.2) & 0.29 & 4.89 & 9.56
\\
Kepler-1390 & 2086485186737501696 & 298.6624 & 48.2488 & 0.735 & -62.7$^{\S}$ & -0.17 & 5392 & 4.21 & TD (a) & 1.61 & -1.56 & 0.31 & (89.8,191.4,-3.89) & 0.19 & 5.04 & 9.71
\\
Kepler-1466 & 2126944603296783232 & 289.8312 & 44.6098 &	0.629 & -99.8$^{\S}$ & -0.51 & 5660 & 4.39 & TD (a) & 1.69 & -1.30 & 0.30 & (21.9,160.8,-40.8) & 0.82 & 4.35 & 8.17
\\
Kepler-1519 &2086851495906130176 & 296.6679 & 49.4617 & 1.492 & -83.2$^{\ddagger}$ & -0.37 & 5467 & 3.90 & TD (b) & 1.62 & -1.50 & 0.25 & (-56.8,183.9,-68.6) & 1.77 & 5.35 & 8.97
\\
Kepler-1559 &2125705488052032640 & 292.2867 & 42.0726 & 0.622 & -85.5$^{\ddagger}$ & 0.07 & 5223 & 4.53 & TD (b) & 1.58 & -1.49 & 0.42 & (130.2,184.6,13.4) & 0.28 & 4.41 & 10.92
\\
Kepler-1619 & 2105921803532722432 & 285.7036 & 44.4222 & 0.736 & -16.7$^{\ddagger}$ & -0.34 & 5634 & 4.18 & TD (b) & 1.36 & -2.13 & 0.48 & (158.9,264.1,-7.0) & 0.53 & 5.97 & 17.19
\\
Kepler-1619 & 2105921803532722432 & 285.7036 & 44.4222	& 0.735 & -25.0$^{\S}$ & -0.29 & 5738 & 4.14 & TD (b) & 1.38 & -2.06 & 0.47 & (160.3,256.0,-9.49) & 0.55 & 5.81 & 16.51
\\
Kepler-1638 & 2134726877877965568 & 295.4823 & 48.5245 & 1.508 & -93.7$^{\ddagger}$ & -0.50 & 5534 & 4.12 & TD (b) & 1.70 & -1.18 & 0.39 & (51.6,144.9,38.3) & 0.86 & 3.66 & 8.50
\\
Kepler-177 & 2106339927188171776 & 286.0471 & 45.0532 & 1.451 & -114.5$^{\ddagger}$ & -0.23 & 5626 & 3.98 & TD (b) & 1.71 & -1.18 & 0.36 & (44.2,148.0,-53.5) & 1.41 & 3.86 & 8.25
\\
Kepler-213 & 2127001056345369984 & 290.8242 & 44.6473 & 0.620 & -82.5$^{\S}$ & 0.11 & 5570 & 4.18 & TD (a) & 1.64 & -1.41 & 0.34 & (83.1,174.9,14.4) & 0.28 & 4.49 & 9.21
\\
Kepler-29 & 2086435189017387264 & 298.3483 & 47.4913 & 0.873 & -59.4$^{\S}$ & -0.63 & 5296 & 4.21 & TD (a) & 1.60 & -1.57 & 0.31 & (90.2,193.1,6.3) & 0.21 & 5.09 & 9.73
\\
Kepler-329 & 2079224424266279936 & 299.2682 & 45.2273 & 0.439 & -102.8$^{\S}$ & -0.46 &	4755 & 4.46 & TD (b) & 1.67 & -1.28 & 0.28 & (-22.2,157.7,-87.6) & 2.28 & 4.71 & 8.38
\\
Kepler-390 & 2101638759069485568 & 291.6288 & 41.2088 & 0.429 & -48.8$^{\ddagger}$ & -0.11 & 5240 & 4.64 & TD (a) & 1.52 & -1.79 & 0.34 & (112.4,220.9,31.5) & 0.68 & 5.70 & 11.51
\\
Kepler-390 & 2101638759069485568 & 291.6288 & 41.2088 & 0.429 & -60.0$^{\S}$ & -0.09 & 5178 & 4.53 & TD (a) & 1.54 & -1.70 & 0.35 & (114.9,210.4,29.3) & 0.61 & 5.36 & 11.1
\\
Kepler-392 & 2102948483573807616 & 288.6608 & 43.3682 & 0.685 & -73.7$^{\S}$ & -0.70 & 5873 & 4.09 & TD (a) & 1.57 & -1.61 & 0.35 & (111.8,200.0,-14.5) & 0.39 & 5.06 & 10.5
\\
Kepler-461 & 2126801563705846528 & 292.2491 & 46.1648 & 0.691 & -111.0$^{\ddagger}$ & -0.11 & 5769 & 4.38 & TD (b) & 1.72 & -1.19 & 0.36 & (-2.7,146.3,-45.2) & 0.94 & 3.82 & 8.13
\\
Kepler-461 & 2126801563705846528 & 292.2491 & 46.1648 & 0.691 & -117.1$^{\S}$ & -0.30 & 5681 & 4.07 & TD (b) & 1.72 & -1.13 & 0.38 & (-1.9,139.9,-46.6) & 0.98 & 3.60 & 8.13
\\
Kepler-611 &2106443453079518336 & 286.0049 & 45.4803 & 1.373 & -36.8$^{\ddagger}$ & 0.12 & 5554 & 3.99 & TD (a) & 1.57 & -1.64 & 0.33 & (-105.6,205.1,-14.3) & 0.56 & 5.25 & 10.47
\\
Kepler-646 & 2126970579257130112 & 290.4715 & 44.3870 & 0.459 & -98.2$^{\S}$ & -0.47 & 5439 & 4.40 & TD (b) & 1.67 & -1.37 & 0.26 & (29.0,169.0,-59.8) & 1.37 & 4.83 & 8.28
\\
Kepler-660 & 2130882023153533184 & 288.1383 & 47.7246 & 0.564 & -95.9$^{\ddagger}$ & -0.27 & 4684 & 4.61 & TD (a) & 1.68 & -1.32 & 0.36 & (72.2,162.6,-6.7) & 0.23 & 4.14 & 8.87
\\
Kepler-749 & 2076090506891080704 & 299.8973 & 43.9041 & 0.750 & -53.2$^{\S}$ & -0.65 & 4868 & 4.29 & TD (b) & 1.50 & -1.68 & 0.44 & (147.9,207.8,25.9) & 0.55 & 4.90 & 12.69
\\
Kepler-966 & 2087263361789975040 & 297.2705 & 50.1218 & 1.042 & -88.8$^{\ddagger}$ & -0.10 & 5646 & 4.21 & TD (a) & 1.70 & -1.29 & 0.33 & (28.2,157.6,12.3) & 0.31 & 4.16 & 8.29
\\
NGTS-4 & 2891248292906892032 & 89.5988 & -30.8118 & 0.277 & 110.4$^{\dagger}$ & & &  & TD (a)
& 1.65 & -1.45 & 0.25 & (32.9,173.6,-59.9) & 1.42 & 5.14 & 8.59
\\
NGTS-4 & 2891248292906892032 & 89.5988 & -30.8118 & 0.277 & 111.6$^{\star}$ & -0.17 & 5135 & 4.49 & TD (a) & 1.65 & -1.45 & 0.25 & (33.4,173.1,-60.3) & 1.43 & 5.11 & 8.60
\\
WASP-4 & 6535499658122055552 & 353.5629 & -42.0618 & 0.272 & 58.8$^{\dagger}$ & & &  & TD (b)
& 1.72 & -1.10 & 0.44 & (-58.7,135.5,-25.9) & 0.53 & 3.27 & 8.23
\\
XO-2 N & 934346809278715776 & 117.0268 & 50.2251 & 0.150 & 47.7$^{\dagger}$ & & &  & TD (a)
& 1.67 & -1.32 & 0.37 & (69.0,158.7,-1.2) & 0.10 & 4.11 & 9.02
\\
XO-2 N & 934346809278715776 & 117.0268 & 50.2251 & 0.150 & 47.1$^{\ddagger}$ & 0.36 & 5160 & 4.27 & TD (a) & 1.67 & -1.32 & 0.37 & (68.5,158.6,-1.43) & 0.10 & 4.11 & 9.01
\\
XO-2 S & 934346740559239296 & 117.0310 & 50.2169 & 0.150 & 46.8$^{\dagger}$ & & &  & TD (a)
& 1.67 & -1.32 & 0.37 & (68.0,158.7,-1.3) & 0.10 & 4.11 & 9.02
\end{longtable}
\end{ThreePartTable}
\end{longrotatetable}
%\end{landscape}

